Evidence of rescattering effect in Pb-Pb collisions at the LHC through production of $\rm{K}^{*}(892)^{0}$ and $\phi(1020)$ mesons

Measurements of $\rm{K}^{*}(892)^{0}$ and $\phi(1020)$ resonance production in Pb-Pb and pp collisions at $\sqrt{s_{\rm{NN}}}$ = 5.02 TeV with the ALICE detector at the Large Hadron Collider are reported. The resonances are measured at midrapidity ($|y|$ $<$ 0.5) via their hadronic decay channels and the transverse momentum ($p_{\rm{T}}$) distributions are obtained for various collision centrality classes up to $p_{\rm{T}}$ $=$ 20 GeV$/c$. The $p_{\rm{T}}$-integrated yield ratio $\rm{K}^{*}(892)^{0}$$/$K in Pb-Pb collisions shows significant suppression relative to pp collisions and decreases towards more central collisions. In contrast, the $\phi(1020)$$/$K ratio does not show any suppression. Furthermore, the measured $\rm{K}^{*}(892)^{0}$$/$K ratio in central Pb-Pb collisions is significantly suppressed with respect to the expectations based on a thermal model calculation, while the $\phi(1020)$$/$K ratio agrees with the model prediction. These measurements are an experimental demonstration of rescattering of $\rm{K}^{*}(892)^{0}$ decay products in the hadronic phase of the collisions. The $\rm{K}^{*}(892)^{0}$$/$K yield ratios in Pb-Pb and pp collisions are used to estimate the time duration between chemical and kinetic freeze-out, which is found to be $\sim$ 4-7 fm$/c$ for central collisions. The $p_{\rm{T}}$-differential ratios of $\rm{K}^{*}(892)^{0}$$/$K, $\phi(1020)$$/$K, $\rm{K}^{*}(892)^{0}$$/\pi$, $\phi(1020)$$/\pi$, $p/$$\rm{K}^{*}(892)^{0}$ and $p/$$\phi(1020)$ are also presented for Pb-Pb and pp collisions at $\sqrt{s_{\rm{NN}}}$ $=$ 5.02 TeV. These ratios show that the rescattering effect is predominantly a low-$p_{\rm{T}}$ phenomenon.

==> abstractcds.tex <==
Measurements of $\rm{K}^{*}(892)^{0}$ and $\phi(1020)$ resonance production in Pb-Pb and pp collisions at $\sqrt{s_{\rm{NN}}}$ = 5.02 TeV with the ALICE detector at the Large Hadron Collider are reported. The resonances are measured at midrapidity ($|y|$ $<$ 0.5) via their hadronic decay channels and the transverse momentum ($p_{\rm{T}}$) distributions are obtained for various collision centrality classes up to $p_{\rm{T}}$ $=$ 20 GeV$/c$. The $p_{\rm{T}}$-integrated yield ratio $\rm{K}^{*}(892)^{0}$$/$K in Pb-Pb collisions shows significant suppression relative to pp collisions and decreases towards more central collisions.
In contrast, the $\phi(1020)$$/$K ratio does not show any suppression. Furthermore, the measured $\rm{K}^{*}(892)^{0}$$/$K ratio in central Pb-Pb collisions is significantly suppressed with respect to the expectations based on a thermal model calculation, while the $\phi(1020)$$/$K ratio agrees with the model prediction. These observations are an experimental 
demonstration of rescattering of $\rm{K}^{*}(892)^{0}$ decay products in the hadronic phase of the collisions. The $\rm{K}^{*}(892)^{0}$$/$K  
yield ratios in Pb--Pb and pp collisions 
are used to estimate the time duration between chemical and kinetic 
freeze-out, which is found to be $\sim$ 4-7 fm$/c$ for central collisions. The $p_{\rm{T}}$-differential ratios of $\rm{K}^{*}(892)^{0}$$/$K, 
$\phi(1020)$$/$K, $\rm{K}^{*}(892)^{0}$$/\pi$, $\phi(1020)$$/\pi$, $p/$$\rm{K}^{*}(892)^{0}$ and $p/$$\phi(1020)$ are also presented for Pb-Pb and pp collisions at $\sqrt{s_{\rm{NN}}}$ $=$ 5.02 TeV. These ratios show that the rescattering effect is predominantly a low-$p_{\rm{T}}$ phenomenon. 
The ratios at intermediate $p_{\rm{T}}$ show the effect of larger radial flow in central Pb--Pb collisions relative to peripheral and 
pp collisions. However, at higher $p_{\rm{T}}$, the ratios for the various collision systems are consistent among each other, confirming that particle production via fragmentation is not significantly modified in the presence of a medium.

